The instantaneous mass accretion rate of novae in quiescence: - an archival ultraviolet optical spectral analysis

Based on archival spectra, we derive the quiescent instantaneous mass transfer rates in novae using synthetic disk spectra generated with tlusty, Gaia parallax-derived distances, and updated color excess values. Our results for nine novae, based on ultraviolet spectra and on a number of optical spectra, yield mass accretion rates that are higher than those derived from simple integration of the UV and optical luminosity. HR Del, 20 years after its eruption, has a mass transfer rate of $4\times 10^{-7}M_\odot$/yr, and is likely burning the accreting H-rich material. V842 Cen, thought to be a low mass transfer system, has a comparable mass accretion rate. For both novae, the enhanced mass transfer must be self-sustained by a feedback loop. RR Pic, with $\dot{M}\approx 5\times 10^{-8}M_\odot$/yr, is better fitted with an accretion disk where the outer region is heated up to 12,000 K, in agreement with H and He emission lines coming from the outer disk and a large emission region on the leading side of the disk. Such a heated disk also gives a good fit to the spectra of CP Lac, and DI Lac with $\dot{M}\sim4.5$ and $9\times 10^{-9}M_\odot$/yr. V1974 Cyg and V533 Her, with an accretion rate of $\sim 3\times 10^{-9}M_\odot$/yr, have a rather flat spectrum. V446 Her and BK Lyn, caught in a state of low accretion, have the lowest mass accretion rates with $\dot{M} \sim 10^{-9}$ and $\sim 10^{-10}M_\odot$/yr respectively. The higher mass transfer rate systems, with $\dot{M}\approx \sim 10^{-7}M_\odot$/yr, agree with the standard disk model; the remaining systems are better fitted when the outer disk is heated to $\sim 12,000$~K. We suggest that irradiation from the heated WD, inner disk, together with tidal interaction, the bright spot, and material overflowing the disk edge, can increase the temperature of the outer disk.

==> abstract.tex <==


We present the first results of our archival spectral analysis 
to derive the quiescent instantaneous mass transfer rates $\dot{M}$ in novae, 
using synthetic disk spectra generated with \textsc{tlusty},   
white dwarf (WD) masses estimates from the literature, Gaia parallax-derived distances, 
and updated color excess values. 
Our results for nine novae, based on ultraviolet spectra and on a number of optical spectra,
yield mass accretion rates that are higher than those derived from simple integration of the UV and optical luminosity. 

Twenty one years after its eruption, HR Del, with a mass transfer rate of $4 \times 10^{-7}M_\odot$/yr,   
must have been burning the H-rich material as it accreted onto the WD.   
V842 Cen, which was previously thought to be a low mass transfer system, happened to be on 
the other extreme with $\dot{M}$ of the order of $10^{-7}M_\odot$/yr.   
For both novae, the enhanced mass transfer rate must have been self-sustained by a feedback loop.   
RR Pic, with $\dot{M}\approx 3 \times 10^{-8}M_\odot$/yr, was better fitted with an accretion
disk in which the outer disk is heated up to a temperature of 12,000~K, in agreement with 
H and He emission lines coming from the outer disk and a large emission region on the leading side 
of the disk. Such a disk, augmented with a heated outer disk, also gives a good fit to the spectra of 
CP Lac, and DI Lac with $\dot{M} \sim4.5$ and $9 \times 10^{-9} M_\odot$/yr.  
V1974 Cyg and V533 Her, with an accretion rate of $\sim 3 \times 10^{-9}M_\odot$/yr, 
have an even flatter spectrum. 
As to V446 Her and BK Lyn, they were caught in a state of low accretion and have  
the lowest mass accretion rates in our sample: $\dot{M} \sim 10^{-9}$ and $\sim 10^{-10}M_\odot$/yr respectively. 

We find the higher mass transfer rate systems, with $\dot{M} \approx \sim 10^{-7}M_\odot$/yr, agree with the standard disk
model, while the remaining systems, with $\dot{M}$ of the order of $10^{-8}M_\odot$/yr and lower,  
are better fitted when the outer disk is heated to $\sim 12,000$~K. 
We suggest that irradiation from the heated WD and inner disk, together with tidal interaction, the bright spot, 
and material overflowing the disk edge and falling back onto the disk near phase 0.5,     
can increase the temperature of the outer disk to $\sim 12,000$~K. The relative contribution of this component  
to the UV and optical spectra increases with decreasing accretion rate. 





\section{\bf Discussion and Conclusions} 


HR Del, T Pyx and V842 Cen, only 10-20 years post eruption,
have the highest mass accretion rate ($\sim 10^{-7}M_\odot$/yr),   
while BK Lyn, $\sim$2000 years after its eruption, has the lowest mass accretion rate
($\sim 10^{-10} M_\odot$/yr). Together with RR Pic, DI Lac and CP Lac, $\sim 70$ years
post-eruption, with an intermediate mass accretion ($\sim 10^{-8}M_\odot$/yr), these 
seven systems seem to hint at a declining $\dot{M}$ with time after nova eruption. 
This, however, certainly needs to be confirmed with many more data points, especially
that the STIS spectrum of BK Lyn was obtained when it was in a low state similar to 
a quiescent DN (see \S 3.1).

For HR Del, the large mass accretion we derived leads to stable burning on the WD surface
(self-sustained feedback loop SSS phase), 
and possibly at a rate slower than the matter is accreted. 
It must form a red giant-like structure or it must be carried away in a wind (see e.g. Fig.2 in \citet{cho21}).  
For T Pyx, the self-sustained feedback loop is shutting down as its accretion rate has been declining for 
the last $\sim$135 years \citep{sch10b,god24}. 
For V842 Cen, by evaluating the color excess from its IUE spectrum, we have now added it to the list 
of self-sustained high accreting novae.
It is clear that these three high accreting novae are distinct from novae like V533 Her 
and V1975 Cyg, which have a mass accretion of only a few $10^{-9}M_\odot$/yr less than 2 decades after
their nova eruption. 

A comparison with the previous analyses of \citet{moy03}, \citet{pue07}, and \citet{sio17} cannot be made
as they assumed different distances, $E(B-V)$ values, and WD masses. 
We are thus left to compare our results with those of \citet{sel19} for the six systems
we have in common. 
For that purpose, we compare the results we obtained with the results of \citet{sel19} 
with a WD mass of $1.0M_\odot$ (column 6, in their Table 2), since our WD 
masses are all nearly solar. 
For V533 Her and V446 Her, we obtained accretion rates that are only slightly larger (by $\sim20$\%). 
For DI Lac and CP Lac, we obtained accretion rates twice as large, however, the analysis
of the optical spectrum of CP Lac yielded the same accretion rate as \citet{sel19}. 
For RR Pic, we obtained an accretion rate three times larger. 
For HR Del, we adopted a WD mass very close to that of \citet{sel19} and obtained 
an accretion rate five times larger. 

As mentioned earlier in \S1, the mass accretion rates derived using the standard disk model
\citep[i.e. with {\textsc{tlusty};}][]{pue07} are on average 3 times larger than derived based on the observed
UV and optical luminosity \citep{gil24}. We notice that the largest discrepancy we obtained 
with \citet{sel19} is for HR Del, which has a spectrum that best agrees with 
a standard disk model. For the remaining five novae in common, the outer region of the disk was assumed
to have a temperature of $\sim 12,000$~K. That large outer region provided additional flux
and therefore, the resulting mass accretion rate was lower than for the standard disk model,
in better agreement with the results of \citet[][for the $1.0M_\odot$ WD masses]{sel19}.  

In the present work we adopted the WD masses from \citet{sha18}, 
which are larger than the WD masses derived by \citet{sel19} and \citet{hac19}.  
In particular, WD masses smaller than $\sim  1.0-1.1 M_\odot$ in \citet{sel19} and \citet{hac19} 
are on average $\sim 0.2M_\odot$ larger in \citet{sha18}, and the discrepancy
increases with decreasing WD mass. 
The remaining nova WDs larger than $\sim 1.1 M_\odot$ in \citet{sel19} and \citet{hac19}
have on average the same masses in \citet{sha18}. This is explicitly displayed in Figs.\ref{shk}a and b. 


The direct consequence of assuming a larger WD mass is a lower mass accretion rate.
Namely, had we assumed lower WD masses, we would have obtained even larger mass accretion rates. 

To further constrain the WD mass, it is important to consider the following. 
Positive superhumps are believed to be caused by the accretion disk becoming eccentric 
(due to tidal forces from the secondary) and precessing. 
Namely, superhumps are triggered when the outer disk reaches the 3:1 resonance radius, 
implying a small mass ratio $q=M_2/M_1 \le 0.3.$ 
This naturally occurs in systems with a smaller secondary mass below the period gap 
(where $M_2 \le 0.2 M_\odot$, such as for BK Lyn \& V1974 Cyg), 
but above the period gap it implies a large WD primary mass ($\sim 1 M_\odot$).   
RR Pic and V533 Her exhibit positive superhumps \citep{bru22,bru23a,bru23b}, they are therefore expected to have
a large WD mass. 

For four decades already, the validity of the standard $\alpha$-disk model has been questioned,
mainly because disk models, as those generated using \textsc{tlusty}, have systematically disagreed  
with the observations: the continuum of the observed spectra have a shallower slope, or alternatively,
the theoretical spectra are bluer \citep{wad84,wad88}. And while many explanations and solutions have
been advanced, this issue remains a matter of debate \citep[see][and references therein]{zsi24}. 
In the present work, we found that for systems accreting at a very high rate, $\sim 10^{-7}M_\odot$/yr
(as for V842 Cen, HR Del, and T Pyx), the observed spectra are bluer and agree with the standard disk model. 
As the mass accretion rate decreases the observed spectra seem to become flatter, though many other factors
can affect the spectra: e.g. highly inclined systems have flatter spectra; short spectral range spectra
(e.g. from 1200~\AA\ to 1700~\AA ) are easier to fit than large spectra range (e.g. covering UV + optical);
low S/N, and so on. Not unlike the nova-likes BZ Cam and V592 Cas \citep{god17}, we find that the addition of 
an outer disk with a temperature of the order of $\sim 12,000$~K improves the fit. 
If indeed, a $12,000$~K component with a large emitting area is contributing to the 
UV and optical, its relative contribution to the UV and optical flux decreases as $\dot{M}$ increases, 
in agreement with our disk modeling.  

Though our modeling is entirely empirical, there are observational evidence 
and physical processes at work to support the heating of the outer disk.  
The superhumps, mentioned above, through the 3:1 resonance, inject extra energy into the outer disk.  
Tidal interaction, even without the disk reaching the 3:1 resonance, heats up the outer region of the disk,
either through spiral shocks (at higher Mach number/low viscosity/low mass accretion rates) 
or through continuous background shearing due to the non-axisymmetric trajectories
of the gas elements (at low Mach number/high viscosity/high mass accretion rates), 
or through both \citep{ogi02,ju16}. 
The bright spot, that region at the edge of the disk being hit by the L1 stream, is also providing 
additional heating in the outer disk. Even material from the L1 stream overflowing the disk's edge 
will fall back onto the disk near orbital phase $\sim$0.5-0.6 \citep[e.g.][]{lub89,god19} and release 
some of its kinetic energy there. 
As the outer disk heats up, it extends vertically, thereby intercepting more ionizing radiation from the 
hot WD, boundary layer, and/or inner disk, which further increases its temperature. 
And while it is clear that heating of the outer disk takes place during the self-sustained enhanced
accretion phase (since the source irradiating the secondary also irradiates the disk), 
it is also very likely that it takes place at lower mass accretion rates. 
However, the emission from the hot inner (standard) disk itself completely dominates the UV and optical 
when the mass accretion rate is large, and only at lower accretion rates does the contribution of 
the outer disk become apparent. 

We therefore suggest that heating of the outer disk might be responsible, {\it at least in part}, for the shallower
slope of the observed spectra of accreting WDs.  
Geometrical effects, such as self-occultation of the disk, and large stream disk overflow can also 
affect the shape of the continuum making it flatter, as observed e.g. in the STIS spectra of EM Cyg 
\citep[see Figs.1 and 2, lower left panel, in][]{god19}.  

At this stage of our research, we did not check whether the mass accretion rate correlates with the time ($t_3$) it takes
for the nova to fade by 3 magnitudes after its eruption. Our current statistically small number  
of novae is further diminished by the fact that two novae, V446 Her and BK Lyn, were caught in a state of low mass 
accretion. Furthermore, for BK Lyn, the $t_3$ time and the characteristics of its eruption 
are entirely unknown. We have, however, assessed its WD mass as $1.0-1.2 M_\odot$ and have 
put a lower limit on its mass accretion rate $\approx 10^{-10}M_\odot$/yr (quiescent accretion rate). 
For these results, the buildup time to reach an envelope mass capable of triggering
the next nova eruption ranges roughly from $\approx$300,000~yr to $\approx$1 million years. 
Since the accretion rate is the quiescent one, these times are upper limit, assuming of course that
BK Lyn doesn't go into hibernation. Therefore, even 2000~years after its eruption, this might
not reflect its long-term accretion rate between eruptions. 

It is interesting to note that 
the mass accretion rate we found for V446 Her, $6.3 \times 10^{-10} < \dot{M}/(M_\odot$/yr)$ < 2.52 \times 10^{-9}$,  
does not reflect a DN quiescent state with $\dot{M} < 10^{-10}M_\odot$/yr, not an optically thin disk.  
Instead, it is possible that V446 Her might not be reaching a true DN quiescent state, especially
that the `outburst' amplitude is really small, of the order of 1.5 magnitudes. 







